Exact Minkowski Sums of Polygons With Holes

We present an efficient algorithm that computes the Minkowski sum of two polygons, which may have holes. The new algorithm is based on the convolution approach. Its efficiency stems in part from a property for Minkowski sums of polygons with holes, which in fact holds in any dimension: Given two polygons with holes, for each input polygon we can fill up the holes that are relatively small compared to the other polygon. Specifically, we can always fill up all the holes of at least one polygon, transforming it into a simple polygon, and still obtain exactly the same Minkowski sum. Obliterating holes in the input summands speeds up the computation of Minkowski sums. We introduce a robust implementation of the new algorithm, which follows the Exact Geometric Computation paradigm and thus guarantees exact results. We also present an empirical comparison of the performance of Minkowski sum construction of various input examples, where we show that the implementation of the new algorithm exhibits better performance than several other implementations in many cases. In particular, we compared the implementation of the new algorithm, an implementation of the standard convolution algorithm, and an implementation of the decomposition approach using various convex decomposition methods, including two new methods that handle polygons with holes - one is based on vertical decomposition and the other is based on triangulation. The software has been developed as an extension of the "2D Minkowski Sums" package of CGAL (Computational Geometry Algorithms Library). Additional information and supplementary material is available at our project page http://acg.cs.tau.ac.il/projects/rc

==> Makefile <==
LANGUAGE = en_US
DOCUMENTS = main.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	3sat gadget_and gadget_crossing gadget_inverter gadget_multiplexer \
	gadget_or_bb gadget_or_rb gadget_variable needles three_colorability, \
	graphics/$g.pdf_tex)

main.pdf: main.tex llncs.cls header.tex abbrv.bst \
	general.tex fig/trace_ms.pdf fig/trace_p.pdf \
	abstract.tex \
	introduction.tex \
	implementation.tex \
	experiments.tex \
        fig_convolution_with_hole.tex \
	bibliography.bib abrev.bib
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS)
	rm -f *.aux *.bbl *.blg *.log *.out
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)


==> decomposition.tex <==
% =============================================================================
\section{Decomposition approach}
\label{sec:decomposition}
% =============================================================================

Calculating the Minkowski sum of two convex polygons is rather easy
using an operation similar to the merge step of the merge-sort
algorithm, as $P \oplus Q$ is a convex polygon bounded by copies of
the edges of $P$ and $Q$ ordered according to the angle they form with
the $x$-axis.

So, decompose $P$ and $Q$ into convex sub-polygons, namely obtain two sets
of convex polygons $P_1, \ldots, P_k$ and $Q_1, \ldots, Q_\ell$ such
that $\bigcup_{i = 1}^{k}{P_i} = P$ and $\bigcup_{i = j}^{\ell}{Q_j} =
Q$.  Then, calculate the pairwise sums $S_{ij} = P_i \oplus Q_j$ using
the simple procedure described above, and compute the union
$P \oplus Q = \bigcup_{ij}{S_{ij}}$.

\todo[inline]{Describe the new decomposition methods.}


==> fig_convolution.tex <==
\def\convA{%
  \begin{tikzpicture}[scale=0.35]
    \filldraw[color=polyADarkColor,fill=polyALightColor,thick]%
    (1.5,0)--(0,1.5)--(-1.5,0)--(0,-1.5)--cycle;
  \end{tikzpicture}}
\def\convB{%
  \begin{tikzpicture}[scale=0.35]
    \filldraw[color=polyBDarkColor,fill=polyBLightColor,thick]%
    (0,0)--(9,0)--(9,6)--(5,6)--(8,1)--(1,1)--(4,6)--(0,6)--cycle;
  \end{tikzpicture}}
\def\convC{%
  \begin{tikzpicture}[scale=0.35]
    \fill[polyCLightColor]%
    (9,7.5)--(5,7.5)--(4.5,7)--(4,7.5)--(0,7.5)--(-1.5,6)--(-1.5,0)--(0,-1.5)--(9,-1.5)--(10.5,0)--(10.5,6)--cycle;
    \fill[white](5.6,2.5)--(3.4,2.5)--(4.5,4.33333)--cycle;
    \draw[black,thick,->](9,7.5)--(5,7.5);
    \draw[black,thick,->](5,7.5)--(3.5,6);
    \draw[black,thick,->](3.5,6)--(6.5,1);
    \draw[black,thick,->,dotted](6.5,1)--(8,-0.5);
    \draw[black,thick,->,dotted](8,-0.5)--(9.5,1);
    \draw[black,thick,->,dotted](9.5,1)--(8,2.5);
    \draw[black,thick,->](8,2.5)--(1,2.5);
    \draw[black,thick,->,dotted](1,2.5)--(-0.5,1);
    \draw[black,thick,->,dotted](-0.5,1)--(1,-0.5);
    \draw[black,thick,->,dotted](1,-0.5)--(2.5,1);
    \draw[black,thick,->](2.5,1)--(5.5,6);
    \draw[black,thick,->](5.5,6)--(4,7.5);
    \draw[black,thick,->](4,7.5)--(0,7.5);
    \draw[black,thick,->](0,7.5)--(-1.5,6);
    \draw[black,thick,->](-1.5,6)--(-1.5,0);
    \draw[black,thick,->](-1.5,0)--(0,-1.5);
    \draw[black,thick,->](0,-1.5)--(9,-1.5);
    \draw[black,thick,->](9,-1.5)--(10.5,0);
    \draw[black,thick,->](10.5,0)--(10.5,6);
    \draw[black,thick,->](10.5,6)--(9,7.5);
    \node at (4.5,3.2) {$[0]$};
    \node at (10.2,7.2) {$[0]$};
    \node at (4.5,0.5) {$[1]$};
    \node at (1,1) {$[2]$};
    \node at (8,1) {$[2]$};
    \node at (4.5,5.85) {$[2]$};
  \end{tikzpicture}}


\begin{figure}[ttp]
  \setlength{\tabcolsep}{2pt}
  \centering
  \begin{tabular}{lr}
    \convA&\multirow{2}*[24pt]{\convC}\\
    \convB&\\
  \end{tabular}
\caption[The convolutions of a convex and a concave polygons]{
  The convolution of a convex and a non-convex polygon;
  winding numbers are indicated in brackets;
  dotted edges are left out for the reduced convolution.
  %  The convolution of a convex and a non-convex polygon, which consists of
  %  a single self-intersecting cycle, drawn as a chain of directed line
  %  segments. The winding numbers of the faces of the arrangement
  %  induced by the segments forming the cycle are indicated in
  %  brackets. The Minkowski sum of the two polygons is shaded.
  }
  \label{fig:onecyc}
\end{figure}

\ignore{
\begin{figure}[ttp]
  %\setlength{\tabcolsep}{0pt}
  \centering
  \begin{tabular}{p{\linewidth}}
    \begin{tabular*}{\linewidth}{l@{\extracolsep{\fill}}r}
      \convA & \convB
    \end{tabular*}\tabularnewline
    \begin{tabular*}{\linewidth}{l@{\extracolsep{\fill}}r}
      (a) The convex polygon. & (b) The concave polygon.\tabularnewline
    \end{tabular*}\tabularnewline
    \multicolumn{1}{c}{\convC}\tabularnewline
    \multicolumn{1}{c}{(c) The convolution and Minkowski sum.}
  \end{tabular}



%%   \subfloat[][The convex polygon.]{\convA}\hfill
%%   \subfloat[][The concave polygon.]{\convB}\hfill
%%   \subfloat[][The convolution cycle and the winding numbers it induces.]{\convC}
  \caption[The convolutions of a convex and a concave polygons]{
    The convolution of a convex and a non-convex polygon;
    winding numbers are indicated in brackets;
    dotted edges are not part of the reduced convolution.
%  The convolution of a convex and a non-convex polygon, which consists of
%  a single self-intersecting cycle, drawn as a chain of directed line
%  segments. The winding numbers of the faces of the arrangement
%  induced by the segments forming the cycle are indicated in
%  brackets. The Minkowski sum of the two polygons is shaded.
  }
  \label{fig:onecyc}
\end{figure}
}


==> old/general_efi.tex <==
% =============================================================================
\section{Filtering Out Holes}
\label{sec:filtration}
% =============================================================================
The fundamental observation of the convolution theorem is that only
points on the boundary of $P$ and $Q$ can contribute to the boundary
of $P\oplus Q$. Specifically, the set of segments in the convolution
$P*Q$ is a superset of the segments of the boundary of $P\oplus Q$.

The idea behind the reduced convolution method is to filter out
segments of $P*Q$ that can not possibly contribute to the boundary of
$P\oplus Q$ using a local criterion; see Section~\ref{ssec:terms}.  In
this section we introduce a global criterion. We show that if a hole
in one polygon is relatively small compared to the other polygon, the
hole is irrelevant for the computation of $P\oplus Q$. Thus, we can
ignore all segments in $P*Q$ that are induced by the hole when
computing $P\oplus Q$. It implies that the hole can be removed (that
is, filled up) before the main computation starts, regardless of the
used approach; see also Figure~\ref{fig:path_and_hole} for an
intuition.

\begin{figure}[htb]
\center
\includegraphics[width=0.7\columnwidth]{./ipe/sum_path_hole.pdf}
\caption{\cpationstyle%
  A small hole $H$ is irrelevant for the computation of $P\oplus Q$
  as adding $\partial H$ and $\gamma \subset Q$ fills up any potential hole
  in $P\oplus Q$ related to $H$.
\label{fig:path_and_hole}}
\end{figure}

\begin{definition}
  A hole $H$ of polygon $P$ leaves a trace in $P \oplus Q$, if there
  exists a point $r = p+q \in \partial(P \oplus Q)$, such that $p \in
  \partial H$ and $q \in \partial Q$. We say that $r$ is the trace of
  $H$.  Conversely, we say that a hole $H$ is irrelevant for the
  computation of $P \oplus Q$ if it does not leave a trace at all.
\end{definition}

\begin{lemma}\label{lemmaA}
  If $H$ leaves a trace in $P \oplus Q$ at a point $r$, then $r$ is on
  the boundary of a hole $\overline H$ in $P \oplus Q$.
\end{lemma}

\begin{figure}[htb]
  \centering
  \subfloat[][The summand $P$.]{\label{fig:trace::p}
    \includegraphics[width=4cm]{fig/trace_p.pdf}
  }
  \subfloat[][The Minkowski sum $P \oplus Q$]{\label{fig:trace:ms}
    \includegraphics[width=4cm]{fig/trace_ms.pdf}
  }
  \caption{\cpationstyle%
    A Hole $H$ leaves a trace in $P \oplus Q$ at a point $r=p+q$.  The
    neighborhood of $r$ is magnified. It is depicted as a disk bounded
    by a dashed circle.  The point $z_0 \not \in P \oplus Q$ is
    enclosed by the closed curve $\partial H \oplus q$.
    \label{fig:trace}}
\end{figure}

\begin{proof}
  Consider the point $r = p+q$, which is on the boundary of $P \oplus
  Q$. Since the polygons are closed, for every neighborhood of $r$
  there exists a point $z_0 \not \in P \oplus Q$, which is also inside
  $H \oplus q$; see Figure \ref{fig:trace}. Observe that a point in
  the gray area in the figure must be inside $P \oplus Q$; thus, $z_0$
  must be in the complement of the gray area.) As $z_0$ is enclosed by
  the closed curve $\partial H \oplus q \subset P \oplus Q$, $z_0$ is
  inside a hole $\overline H$ in $P \oplus Q$.
\end{proof}

\begin{lemma}\label{lemmaB}
  Let $\overline H$ be a hole in $P \oplus Q$ that contains a point $r
  = p + q \in \partial \overline H$, such that $p \in \partial H$ and
  $q \in \partial Q$; that is, $r$ is a trace of $H$. Then $\forall z
  \in \overline H$ and $\forall y \in Q$, it must hold that $z \in H
  \oplus y$. In other words, $\overline H \subseteq H
  \oplus q\,|\,\forall q\in Q$.
\end{lemma}

\begin{proof}
  As in Lemma \ref{lemmaA}, there is a $z_0$ in the neighborhood of
  $r$ which is enclosed by $\partial H \oplus q$. Furthermore, there
  exists a path to any $z$ in $\overline H$, which means that $z$ is
  also enclosed by $\partial H \oplus q$, or in other words: $z \in H
  \oplus q$.

  Now assume for contradiction that there is a point $y_0 \in Q$, for
  which $z$ is not in $H \oplus y_0$.  Now consider the continuous
  path $\gamma$ that connects $q$ and $y_0$ within $Q$.  Observe that
  $z \in H \oplus q$ and $z \notin H \oplus y_0$ are equivalent to $z
  - q \in H$ and $z - y_0 \notin H$, respectively.  This means that $z
  - y_0$ is either in the unbounded face, or in some other hole of
  $P$.  Now observe that the path $z \oplus (-\gamma)$ connects $z -
  q$ and $z - y_0$.  There must be a point $y_0' \in \gamma \subset
  Q$, for which $z - y_0' \in P$, since $\gamma$ is continuous.
  Hence, $z \in P \oplus y_0'$, which implies $z \in P \oplus Q$---a
  contradiction.
\end{proof}

\begin{theorem}\label{theorem1}
  Let $H$ be a closed hole in polygon $P$. If there is a path
  contained in polygon $Q$ that does not fit under any translation
  in~$-H$, then $H$ is irrelevant for the computation of $P\oplus Q$.
\end{theorem}

\begin{proof}
  Let $\gamma$ be a path contained in polygon $Q$, such that it does
  not fit under any translation in~$-H$.  Assume for contradiction
  that $H$ leaves a trace in $P \oplus Q$; that is, there is an $r = p
  + q \in \partial (P \oplus Q)$, such that $p\in\partial H$ and $q
  \in \partial Q$.  By Lemma~\ref{lemmaB}, for any point $x \in
  \overline H$ it must hold that $x \in H \oplus y$ $\forall y\in Q$.
  Specifically, it must hold $\forall y \in \gamma \subset Q$.  This
  is equivalent to $y \in (x \oplus -H)$ for all $y\in \gamma$,
  stating that $\gamma$ fits into $-H$ under some translation---a
  contradiction.
\end{proof}

The other direction also holds:

\begin{theorem}\label{theorem2}
  Let $H$ be a hole in polygon $P$. If all paths contained in polygon
  $Q$ fit in $-H$ under some translation, then $H$ is relevant for the
  computation of $P\oplus Q$; that is, $P \oplus Q \ne P' \oplus Q$
  with $P' = P \cup H$.
\end{theorem}

\begin{proof}
  If all paths contained in $Q$ fit in $-H$, the path along the outer
  boundary of $Q$ does too.  This means that $Q$ itself fits in $-H$
  under some translation $x$ with $x \oplus Q \subseteq -H$.  In this
  case $x+q \in -H\,|\,\forall q \in Q$, which is equivalent to $-x \in
  H \oplus q\,|\,\forall q \in Q$. As $-x$ is inside $H$ for each
  possible translation of $P$, this implies that $-x \notin P \oplus
  Q$. But at the same time, $-x$ is inside each possible translation
  of $P'$, so $-x \in P \oplus Q$.
\end{proof}

\begin{corollary}\label{cor:hole_filter}
  If the closed axis-aligned bounding box $B_Q$ of $Q$ does not fit
  under any translation in the open axis-aligned bounding box
  $\mathring B_H$ of a hole $H$ in $P$, then $H$ does not have a trace
  in $P \oplus Q$.
\end{corollary}

\begin{proof}
  \Obda assume that $B_Q$ does not fit into $B_H$ with respect to the
  $x$-direction. Consider the two extreme points on $\partial Q$ in
  that direction and connect them by a closed path $\gamma$, which
  obviously does not fit into $-H$, as it does not fit into $B_H$.
\end{proof}

Note that if $B_Q$ does not fit in the open axis-aligned bounding box
$\mathring B_P$ of $P$, it cannot fit in the bounding box of any hole
of~$P$, implying that all holes of $P$ can be ignored. Since for any
two bounding boxes either $B_Q \not \subset \mathring B_P$ or $B_P
\not \subset \mathring B_Q$ holds, we need to consider the holes of at
most one polygon.

Consequently, we can remove all holes whose bounding boxes are, in
$x$- or $y$-direction, smaller than, or as large as, the bounding box
of the other polygon, as an initial phase of all methods. With fewer
holes, convex decomposition results in fewer pieces. Moreover, when
all holes of a polygon become irrelevant, one can choose a
decomposition method that handles only simple polygons instead of a
decomposition method that handles polygons with holes, which is
typically more costly. As for the convolution approach, the
intermediate arrangements become smaller, speeding up the algorithm.

\ignore{
\begin{definition}
A hole $H$ of polygon $P$ is \emph{irrelevant} to the Minkowski sum
$P\oplus Q$ if no point on $\partial H$ contributes to a point on
$partial(P\oplus Q)$.
\end{definition}

\todo[inline]{I am not happy with the following version of the proof
  as $\overline H$ is not motivated clearly. Specifically, why would a
  boundary of H not contribute to the outer boundary of the MS?}

\begin{proof}
Assume to the contrary that there is a hole $H$ in $P$ that is
relevant (namely, not irrelevant) to $P\oplus Q$ but there is a path
$\gamma\in Q$ that does not fit inside $-H$ under any
translation. Since $H$ is relevant there must be a hole $\overline{H}$
in $\partial H\oplus Q$.  Let $x$ be a point inside $\overline{H}$,
then Then $x\in{\it int}(H)\oplus y\ \forall y \in Q$.  Specifically,
it must hold $\forall y \in \gamma \subset Q$.  This is equivalent to
$y \in (x \oplus -H)$ for all $y\in \gamma$, stating that $\gamma$
fits into $-H$ under some translation---a contradiction.
\end{proof}
}

